Mind Meets Robots: A Review of EEG-Based Brain-Robot Interaction Systems

Brain-robot interaction (BRI) empowers individuals to control (semi-)automated machines through their brain activity, either passively or actively. In the past decade, BRI systems have achieved remarkable success, predominantly harnessing electroencephalogram (EEG) signals as the central component. This paper offers an up-to-date and exhaustive examination of 87 curated studies published during the last five years (2018-2023), focusing on identifying the research landscape of EEG-based BRI systems. This review aims to consolidate and underscore methodologies, interaction modes, application contexts, system evaluation, existing challenges, and potential avenues for future investigations in this domain. Based on our analysis, we present a BRI system model with three entities: Brain, Robot, and Interaction, depicting the internal relationships of a BRI system. We especially investigate the essence and principles on interaction modes between human brains and robots, a domain that has not yet been identified anywhere. We then discuss these entities with different dimensions encompassed. Within this model, we scrutinize and classify current research, reveal insights, specify challenges, and provide recommendations for future research trajectories in this field. Meanwhile, we envision our findings offer a design space for future human-robot interaction (HRI) research, informing the creation of efficient BRI frameworks.

==> Big_table.tex <==
\begin{table*}
\footnotesize
\newcommand*\rot[1]{\hbox to1em{\hss\rotatebox[origin=br]{-48}{#1}}}
\newcommand*\feature[1]{\ifcase#1 {$\times$} \or {$\pmb{\checkmark}$} \or {$\diamond$} \fi}
\newcommand*\fthr[3]{\feature#1&\feature#2&\feature#3}
\newcommand*\four[4]{\feature#1&\feature#2&\feature#3&\feature#4}
\newcommand*\five[5]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5}
\newcommand*\fsix[6]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6}
\newcommand*\fsvn[7]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6&\feature#7}
\newcommand*\feit[8]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6&\feature#7&\feature#8}
\makeatletter
\newcommand*\ex[5]{#1 & #2 & \four#3 & \four#4 & \fsix#5}
\makeatother
\newcolumntype{G}{c@{}c@{}c}
\newcolumntype{L}{c@{}c@{}c@{}c}
\newcolumntype{H}{c@{}c@{}c@{}c@{}c@{}c}
\newcolumntype{J}{c@{}c@{}c@{}c@{}c@{}c@{}c}
\newcolumntype{K}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}

\caption{The overview of the BRI model with respect to the three entities identified in our corpus, which addresses the relevance between the dedicated dimensions and each individual paper. {$\pmb{\checkmark}$}: completely relevant; {$\times$}: not relevant; {$\diamond$}: relevant either indirectly, implicitly, or partially. Note: the {$\diamond$} mark denoted in signal acquisition, preprocessing, feature extraction, and feature classification represent that these dimensions lacked detailed descriptions in the reviewed papers. Cont. next page.}
\label{tab:everything}
\begin{tabular}{@{}ll !{\kern1.5em} L !{\kern1.5em} L !{\kern2em} H@{}}
\specialrule{.2em}{.1em}{.1em}
\toprule
\multicolumn{2}{l}{LITERATURE} &
\multicolumn{4}{c}{\hspace*{-2cm}BRAIN} & 
\multicolumn{4}{c}{\hspace*{-0.8cm}INTERACTION} & 
\multicolumn{6}{c}{ROBOT} \\ 

\midrule
\midrule

&
& \rot{Signal Acquisition}
& \rot{Prepossessing}
& \rot{Feature Extraction}
& \rot{Feature Classification}
%
& \rot{\textbf{Pure BCI}}
& \rot{\textbf{Auxiliary BCI}}
& \rot{\textbf{Proactive Control}}
& \rot{\textbf{Tasking HRI}}

%
& \rot{Robot Arm}
& \rot{Mobile Robot}
& \rot{Humanoid Robot }
& \rot{Wearable Robot}
& \rot{Social Robot}
& \rot{Drone}

\\
\midrule
\ex{\cite{qian2018affective}}                            {Qian et al 2018}                  {1111} {0001} {100000} \\
\ex{\cite{ogino2018eeg}}                            {Ogino et al 2018}                      {1111} {0010} {100000} \\
\ex{\cite{chu2018robot}}                                 {Chu et al 2018}                    {1111} {1010} {200100} \\
\ex{\cite{kilmarx2018sequence}}                         {Kilmarx et al 2018}                 {1120} {1010} {100000} \\
\ex{\cite{wang2018study}}                                 {Wang et al 2018}                  {1110} {1010} {010000} \\
\ex{\cite{cao2018tactile}}                                  {Cao et al 2018}                 {1112} {1010} {100000} \\
\ex{\cite{penaloza2018android}}                      {Penaloza et al 2018}                   {2112} {1001} {001000} \\
\ex{\cite{xu2018eeg}}                                    {Xu et al 2018}                     {2011} {0010} {100000} \\
\ex{\cite{kompatsiari2018}}                              {Kompatsiari et al 2018}           {1120} {0001} {001000} \\
\ex{\cite{si2018towards}}                               {Si-Mohammed et al 2018}             {1111} {1111} {010000} \\
\ex{\cite{kuffuor2018brain}}                      {Kuffuor et al 2018}                       {1111} {0110} {010000} \\
\ex{\cite{yuan2018brain}}                          {Yuan et al 2018}                         {1121} {0110} {010000} \\
\ex{\cite{jiang2018brain}}                        {Jiang et al 2018}                         {1111} {1010} {001000} \\
\ex{\cite{wang2018continuous}}                    {Wang et al 2018}                          {1111} {0110} {100000} \\
\ex{\cite{ai2018cooperative}}                        {Ai et al 2018}                         {2212} {0110} {000100} \\
\ex{\cite{memar2018eeg}}                               {Memar et al 2018}                   {1110} {1010} {100000} \\
\ex{\cite{hernandez2019deep}}                        {Hernandez et al 2019}                  {1110} {0010} {100000} \\
\ex{\cite{yu2019design}}                              {Yu et al 2019}                        {1120} {0001} {010000} \\
\ex{\cite{li2019hybrid}}                              {Li et al 2019}                        {1111} {0110} {000100} \\
\ex{\cite{chiuzbaian2019mind}}                      {Chiuzbaian et al 2019}                  {1112} {1010} {000001} \\
\ex{\cite{bahman2019robot}}                           {Bahman et al 2019}                    {1122} {1010} {001000} \\
\ex{\cite{aznan2019using}}                              {Aznan et al 2019}                   {1221} {0101} {001000} \\
\ex{\cite{ghosh2019continuous}}                         {Ghosh et al 2019}                   {1011} {1010} {000100} \\
\ex{\cite{baka2019talking}}                             {Baka et al 2019}                   {1100} {0001} {001020} \\
\ex{\cite{ehrlich2019feasibility}}                      {Ehrlich et al 2019}                {1111} {2010} {001000} \\
\ex{\cite{braun2019prototype}}                             {Braun et al 2019}               {1121} {1002} {001010} \\
\ex{\cite{aldini2019effect}}                            {Aldini et al 2019}                 {1120} {0011} {120000} \\
\ex{\cite{rahul2019eeg}}                              {Rahul et al 2019}                     {1111} {0010} {010000} \\
\ex{\cite{long2019eeg}}                                  {Long et al 2019}                  {1111} {1111} {000100} \\
\ex{\cite{iwane2019inferring}}                              {Iwane et al 2019}              {1111} {1010} {100000} \\
\ex{\cite{memar2019objective}}                              {Memar et al 2019}              {1111} {0021} {100000} \\
\ex{\cite{korovesis2019robot}}                       {Korovesis et al 2019}                  {2111} {0010} {010000} \\
\ex{\cite{chhabra2020bci}}                               {Chhabra et al 2020}               {1211} {1010} {000001} \\
\ex{\cite{lu2022online}}                                    {Lu et al 2020}                 {1111} {1010} {010000} \\
\ex{\cite{alimardani2020robotM}}                           {Alimardani et al 2020}          {1120} {1001} {001020} \\
\ex{\cite{rashid2020investigating}}                  {Rashid et al 2020}                     {1111} {0110} {010000} \\
\ex{\cite{zhao2020multiple}}                          {Zhao et al 2020}                      {2111} {1010} {100000} \\
\ex{\cite{guo2020nao}}                                {Guo et al 2020}                       {1111} {1010} {001000} \\
\ex{\cite{gordleeva2020real}}                       {Gordleeva et al 2020}                   {1111} {0010} {000100} \\
\ex{\cite{nann2020restoring}}                          {Nann et al 2020}                     {1122} {0010} {000100} \\
\ex{\cite{chen2020combination}}                    {Chen et al 2020}                         {1121} {0110} {100000} \\
\ex{\cite{lu2020tractor}}                              {Lu et al 2020}                       {1111} {0010} {010000} \\

% \ex{\cite{sanguantrakul2020development}}        {Sanguantrakul et al 2020}                   {1211} {1010} {0010000} \\
% \ex{\cite{mondini2020continuous}}                     {Mondini et al 2020}                   {1110} {0010} {1000000} \\
% \ex{\cite{shao2020eeg}}                                {Shao et al 2020}                     {1110} {0010} {0100000} \\
% \ex{\cite{abougarair2021implementation}}           {Abougarair et al 2021}                   {2200} {0110} {1000000} \\
% \ex{\cite{zhang2021mind}}                               {Zhang et al 2021}                   {1121} {0110} {1000000} \\
% \ex{\cite{du2021vision}}                               {Du et al 2021}                       {2221} {0110} {1100000} \\
% \ex{\cite{magee2021system}}                             {Magee et al 2021}                   {1121} {0010} {0100000} \\
% \ex{\cite{roshdy2021machine}}                          {Roshdy et al 2021}                   {1221} {1010} {0010000} \\
% \ex{\cite{wei2021control}}                              {Wei et al 2021}                     {2111} {0010} {1000000} \\
% \ex{\cite{araujo2021development}}                    {Araujo et al 2021}                     {1111} {0010} {0000010} \\
% \ex{\cite{ali2021eeg}}                                {Ali et al 2021}                       {1200} {0010} {2000010} \\
% \ex{\cite{francis2021eeg}}                          {Francis et al 2021}                     {2111} {0010} {0100000} \\
% \ex{\cite{belkacem2021cooperative}}                     {Belkacem et al 2021}               {1121} {1010} {0100001} \\
% \ex{\cite{kim2021affect}}                                {Ehrlich et al 2021}               {1122} {0010} {1000000} \\
% \ex{\cite{chang2021eeg}}                                 {Chang et al 2021}                 {1011} {0111} {0100000} \\
% \ex{\cite{toichoa2021emotion}}                          {Toichoa et al 2021}                {1010} {0110} {1000000} \\
% \ex{\cite{wang2021focus}}                               {Wang et al 2021}                   {1120} {1001} {0200100} \\
% \ex{\cite{yoon2021effect}}                              {Yoon et al 2021}                    {1111} {1111} {0010000} \\
% \ex{\cite{liu2021enhanced}}                              {Liu et al 2021}                    {2220} {1010} {0100000} \\
% \ex{\cite{karunasena2021single}}                 {Karunasena et al 2021}                     {1112} {1010} {1000000} \\
% \ex{\cite{kar2021eeg}}                                 {Kar et al 2021}                      {2111} {0100} {1000000} \\
% \ex{\cite{chen2021research}}                              {Chen et al 2021}                  {2211} {0010} {1000000} \\
% \ex{\cite{prinsen2022passive}}                           {Prinsen et al 2022}               {1120} {1001} {0010100} \\
% \ex{\cite{alimardani2022robotL}}                          {Alimardani et al 2022}           {1120} {1001} {0010200} \\
% \ex{\cite{quiles2022cross}}                        {Quiles et al 2022}                       {1111} {1010} {1000000} \\
% \ex{\cite{ak2022motor}}                                {Ak et al 2022}                       {2020} {0110} {1000000} \\
% \ex{\cite{farmaki2022application}}                       {Farmaki et al 2022}               {1111} {1010} {0100000} \\
% \ex{\cite{fang2022brain}}                                   {Fang et al 2022}               {1101} {0110} {1000000} \\
% \ex{\cite{lyu2022coordinating}}                            {Lyu et al 2022}                 {1111} {0110} {1000000} \\
% \ex{\cite{wu2022deepbrain}}                               {Wu et al 2022}                   {2201} {1010} {1000000} \\
% \ex{\cite{dissanayake2022eeg}}                          {Dissanayake et al 2022}            {1110} {1012} {1000000} \\
% \ex{\cite{staffa2022enhancing}}                          {Staffa et al 2022}                {1111} {1002} {0210100} \\
% \ex{\cite{tang2022wearable}}                            {Tang et al 2022}                    {1111} {1111} {0001000} \\
% \ex{\cite{pawus2022application}}                    {Pawus et al 2022}                      {1101} {0010} {0100000} \\
% \ex{\cite{li2022eeg}}                                    {Li et al 2022}                     {2110} {0010} {1000000} \\
% \ex{\cite{roy2022classification}}                       {Roy et al 2022}                     {2121} {0010} {0000010} \\
% \ex{\cite{jo2022eeg}}                                  {Jo et al 2022}                       {1111} {1010} {0001000} \\
% \ex{\cite{aldini2022detection}}                        {Aldini et al 2022}                   {1121} {0001} {1000000} \\
% \ex{\cite{martinez2020non}}                            {Martinez et al 2022}                 {1120} {0010} {1000000} \\
% \ex{\cite{sugiyama2023eeg}}                             {Sugiyama et al 2023}               {2000} {1010} {1000000} \\
% \ex{\cite{richter2023eeg}}                              {Richter et al 2023}                {1112} {0001} {0010200} \\
% \ex{\cite{boonarchatong2023green}}            {Boonarchatong et al 2023}                     {1111} {0010} {1000000} \\
% \ex{\cite{li2023act}}                                       {Li et al 2023}                 {1221} {1010} {0100000} \\
% \ex{\cite{cervantes2023cognidron}}                  {Cervantes et al 2023}                   {1000} {0010} {0000001} \\
% \ex{\cite{chenga2023using}}                             {Chenga et al 2023}                   {1111} {1111} {0010000} \\
% \midrule
% \specialrule{.2em}{.1em}{.1em}
\end{tabular}
\end{table*}

==> Big_table_2.tex <==
\begin{table*}
\footnotesize
\newcommand*\rot[1]{\hbox to1em{\hss\rotatebox[origin=br]{-48}{#1}}}
\newcommand*\feature[1]{\ifcase#1 {$\times$} \or {$\pmb{\checkmark}$} \or {$\diamond$} \fi}
\newcommand*\fthr[3]{\feature#1&\feature#2&\feature#3}
\newcommand*\four[4]{\feature#1&\feature#2&\feature#3&\feature#4}
\newcommand*\five[5]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5}
\newcommand*\fsix[6]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6}
\newcommand*\fsvn[7]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6&\feature#7}
\newcommand*\feit[8]{\feature#1&\feature#2&\feature#3&\feature#4&\feature#5&\feature#6&\feature#7&\feature#8}
\makeatletter
\newcommand*\ex[5]{#1 & #2 & \four#3 & \four#4 & \fsix#5}
\makeatother
\newcolumntype{G}{c@{}c@{}c}
\newcolumntype{L}{c@{}c@{}c@{}c}
\newcolumntype{H}{c@{}c@{}c@{}c@{}c@{}c}
\newcolumntype{J}{c@{}c@{}c@{}c@{}c@{}c@{}c}
\newcolumntype{K}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}

%\begin{longtable}
\caption{Cont.}
\label{tab:everything2}
\begin{tabular}{@{}ll !{\kern1.5em} L !{\kern1.5em} L !{\kern2em} H@{}}
\specialrule{.2em}{.1em}{.1em}
\toprule
\multicolumn{2}{l}{LITERATURE} &
\multicolumn{4}{c}{\hspace*{-2cm}BRAIN} & 
\multicolumn{4}{c}{\hspace*{-0.8cm}INTERACTION} & 
\multicolumn{6}{c}{ROBOT} \\ 
% \multicolumn{6}{c}{DDCs} \\
\midrule
\midrule
% rotated items
&
& \rot{Signal Acquisition}
& \rot{Prepossessing}
& \rot{Feature Extraction}
& \rot{Feature Classification}
%
& \rot{\textbf{Pure BCI}}
& \rot{\textbf{Auxiliary BCI}}
& \rot{\textbf{Proactive Control}}
& \rot{\textbf{Tasking HRI}}

%
& \rot{Robot Arm}
& \rot{Mobile Robot}
& \rot{Humanoid Robot }
% & \rot{Wheeled Robot}
& \rot{Wearable Robot}
% & \rot{Swarm Robot}
& \rot{Social Robot}
% & \rot{Exoskeleton}
& \rot{Drone}

% %
% & \rot{Control Methods}
% & \rot{Flight}
% & \rot{Form}
% & \rot{Lights and Displays}
% & \rot{Proxemics}
% & \rot{Sound}
\\
\midrule
% \ex{\cite{qian2018affective}}                            {Qian et al 2018}                  {1111} {0001} {1000000} \\
% \ex{\cite{ogino2018eeg}}                            {Ogino et al 2018}                      {1111} {0010} {1000000} \\
% \ex{\cite{chu2018robot}}                                 {Chu et al 2018}                    {1111} {1010} {2000010} \\
% \ex{\cite{kilmarx2018sequence}}                         {Kilmarx et al 2018}                 {1120} {1010} {1000000} \\
% \ex{\cite{wang2018study}}                                 {Wang et al 2018}                  {1110} {1010} {0100000} \\
% \ex{\cite{cao2018tactile}}                                  {Cao et al 2018}                 {1112} {1010} {1000000} \\
% \ex{\cite{penaloza2018android}}                      {Penaloza et al 2018}                   {2112} {1001} {0010000} \\
% \ex{\cite{xu2018eeg}}                                    {Xu et al 2018}                     {2011} {0010} {1000000} \\
% \ex{\cite{kompatsiari2018}}                              {Kompatsiari et al 2018}           {1120} {0001} {0010000} \\
% \ex{\cite{si2018towards}}                               {Si-Mohammed et al 2018}             {1111} {1111} {0100000} \\
% \ex{\cite{kuffuor2018brain}}                      {Kuffuor et al 2018}                       {1111} {0110} {0100000} \\
% \ex{\cite{yuan2018brain}}                          {Yuan et al 2018}                         {1121} {0110} {0100000} \\
% \ex{\cite{jiang2018brain}}                        {Jiang et al 2018}                         {1111} {1010} {0010000} \\
% \ex{\cite{wang2018continuous}}                    {Wang et al 2018}                          {1111} {0110} {1000000} \\
% \ex{\cite{ai2018cooperative}}                        {Ai et al 2018}                         {2212} {0110} {0001000} \\
% \ex{\cite{memar2018eeg}}                               {Memar et al 2018}                   {1110} {1010} {1000000} \\
% \ex{\cite{hernandez2019deep}}                        {Hernandez et al 2019}                  {1110} {0010} {1000000} \\
% \ex{\cite{yu2019design}}                              {Yu et al 2019}                        {1120} {0001} {0100000} \\
% \ex{\cite{li2019hybrid}}                              {Li et al 2019}                        {1111} {0110} {0000010} \\
% \ex{\cite{chiuzbaian2019mind}}                      {Chiuzbaian et al 2019}                  {1112} {1010} {0000001} \\
% \ex{\cite{bahman2019robot}}                           {Bahman et al 2019}                    {1122} {1010} {0010000} \\
% \ex{\cite{aznan2019using}}                              {Aznan et al 2019}                   {1221} {0101} {0010000} \\
% \ex{\cite{ghosh2019continuous}}                         {Ghosh et al 2019}                   {1011} {1010} {0000010} \\
% \ex{\cite{baka2019talking}}                             {Baka et al 2019}                   {1100} {0001} {0010200} \\
% \ex{\cite{ehrlich2019feasibility}}                      {Ehrlich et al 2019}                {1111} {2010} {0010000} \\
% \ex{\cite{braun2019prototype}}                             {Braun et al 2019}               {1121} {1002} {0010100} \\
% \ex{\cite{aldini2019effect}}                            {Aldini et al 2019}                 {1120} {0011} {1200000} \\
% \ex{\cite{rahul2019eeg}}                              {Rahul et al 2019}                     {1111} {0010} {0100000} \\
% \ex{\cite{long2019eeg}}                                  {Long et al 2019}                  {1111} {1111} {0000010} \\
% \ex{\cite{iwane2019inferring}}                              {Iwane et al 2019}              {1111} {1010} {1000000} \\
% \ex{\cite{memar2019objective}}                              {Memar et al 2019}              {1111} {0021} {1000000} \\
% \ex{\cite{korovesis2019robot}}                       {Korovesis et al 2019}                  {2111} {0010} {0100000} \\
% \ex{\cite{chhabra2020bci}}                               {Chhabra et al 2020}               {1211} {1010} {0000001} \\
% \ex{\cite{lu2022online}}                                    {Lu et al 2020}                 {1111} {1010} {0100000} \\
% \ex{\cite{alimardani2020robotM}}                           {Alimardani et al 2020}          {1120} {1001} {0010200} \\
% \ex{\cite{rashid2020investigating}}                  {Rashid et al 2020}                     {1111} {0110} {0100000} \\
% \ex{\cite{zhao2020multiple}}                          {Zhao et al 2020}                      {2111} {1010} {1000000} \\
% \ex{\cite{guo2020nao}}                                {Guo et al 2020}                       {1111} {1010} {0010000} \\
% \ex{\cite{gordleeva2020real}}                       {Gordleeva et al 2020}                   {1111} {0010} {0000010} \\
% \ex{\cite{nann2020restoring}}                          {Nann et al 2020}                     {1122} {0010} {0000010} \\
% \ex{\cite{chen2020combination}}                    {Chen et al 2020}                         {1121} {0110} {1000000} \\
% \ex{\cite{lu2020tractor}}                              {Lu et al 2020}                       {1111} {0010} {0100000} \\

\ex{\cite{sanguantrakul2020development}}        {Sanguantrakul et al 2020}                   {1211} {1010} {001000} \\
\ex{\cite{mondini2020continuous}}                     {Mondini et al 2020}                   {1110} {0010} {100000} \\
\ex{\cite{shao2020eeg}}                                {Shao et al 2020}                     {1110} {0010} {010000} \\
\ex{\cite{abougarair2021implementation}}           {Abougarair et al 2021}                   {2200} {0110} {100000} \\
\ex{\cite{zhang2021mind}}                               {Zhang et al 2021}                   {1121} {0110} {100000} \\
\ex{\cite{du2021vision}}                               {Du et al 2021}                       {2221} {0110} {110000} \\
\ex{\cite{magee2021system}}                             {Magee et al 2021}                   {1121} {0010} {010000} \\
\ex{\cite{roshdy2021machine}}                          {Roshdy et al 2021}                   {1221} {1010} {001000} \\
\ex{\cite{wei2021control}}                              {Wei et al 2021}                     {2111} {0010} {100000} \\
\ex{\cite{araujo2021development}}                    {Araujo et al 2021}                     {1111} {0010} {000100} \\
\ex{\cite{ali2021eeg}}                                {Ali et al 2021}                       {1200} {0010} {200100} \\
\ex{\cite{francis2021eeg}}                          {Francis et al 2021}                     {2111} {0010} {010000} \\
\ex{\cite{belkacem2021cooperative}}                     {Belkacem et al 2021}               {1121} {1010} {010001} \\
\ex{\cite{kim2021affect}}                                {Ehrlich et al 2021}               {1122} {0010} {100000} \\
\ex{\cite{chang2021eeg}}                                 {Chang et al 2021}                 {1011} {0111} {010000} \\
\ex{\cite{toichoa2021emotion}}                          {Toichoa et al 2021}                {1010} {0110} {100000} \\
\ex{\cite{wang2021focus}}                               {Wang et al 2021}                   {1120} {1001} {020010} \\
\ex{\cite{yoon2021effect}}                              {Yoon et al 2021}                    {1111} {1111} {001000} \\
\ex{\cite{liu2021enhanced}}                              {Liu et al 2021}                    {2220} {1010} {010000} \\
\ex{\cite{karunasena2021single}}                 {Karunasena et al 2021}                     {1112} {1010} {100000} \\
\ex{\cite{kar2021eeg}}                                 {Kar et al 2021}                      {2111} {0100} {100000} \\
\ex{\cite{chen2021research}}                              {Chen et al 2021}                  {2211} {0010} {100000} \\
\ex{\cite{prinsen2022passive}}                           {Prinsen et al 2022}               {1120} {1001} {001010} \\
\ex{\cite{alimardani2022robotL}}                          {Alimardani et al 2022}           {1120} {1001} {001020} \\
\ex{\cite{quiles2022cross}}                        {Quiles et al 2022}                       {1111} {1010} {100000} \\
\ex{\cite{ak2022motor}}                                {Ak et al 2022}                       {2020} {0110} {100000} \\
\ex{\cite{farmaki2022application}}                       {Farmaki et al 2022}               {1111} {1010} {010000} \\
\ex{\cite{fang2022brain}}                                   {Fang et al 2022}               {1101} {0110} {100000} \\
\ex{\cite{lyu2022coordinating}}                            {Lyu et al 2022}                 {1111} {0110} {100000} \\
\ex{\cite{wu2022deepbrain}}                               {Wu et al 2022}                   {2201} {1010} {100000} \\
\ex{\cite{dissanayake2022eeg}}                          {Dissanayake et al 2022}            {1110} {1012} {100000} \\
\ex{\cite{staffa2022enhancing}}                          {Staffa et al 2022}                {1111} {1002} {021010} \\
\ex{\cite{tang2022wearable}}                            {Tang et al 2022}                    {1111} {1111} {000100} \\
\ex{\cite{pawus2022application}}                    {Pawus et al 2022}                      {1101} {0010} {010000} \\
\ex{\cite{li2022eeg}}                                    {Li et al 2022}                     {2110} {0010} {100000} \\
\ex{\cite{roy2022classification}}                       {Roy et al 2022}                     {2121} {0010} {000100} \\
\ex{\cite{jo2022eeg}}                                  {Jo et al 2022}                       {1111} {1010} {000100} \\
\ex{\cite{aldini2022detection}}                        {Aldini et al 2022}                   {1121} {0001} {100000} \\
\ex{\cite{martinez2020non}}                            {Martinez et al 2022}                 {1120} {0010} {100000} \\
\ex{\cite{sugiyama2023eeg}}                             {Sugiyama et al 2023}               {2000} {1010} {100000} \\
\ex{\cite{richter2023eeg}}                              {Richter et al 2023}                {1112} {0001} {001020} \\
\ex{\cite{boonarchatong2023green}}            {Boonarchatong et al 2023}                     {1111} {0010} {100000} \\
\ex{\cite{li2023act}}                                       {Li et al 2023}                 {1221} {1010} {010000} \\
\ex{\cite{cervantes2023cognidron}}                  {Cervantes et al 2023}                   {1000} {0010} {000001} \\
\ex{\cite{chenga2023using}}                             {Chenga et al 2023}                   {1111} {1111} {001000} \\
% \midrule
% \specialrule{.2em}{.1em}{.1em}
\end{tabular}

% \begin{tablenotes}
% % \item \hfil C: Communication, Control, and Comfort; N: Navigation, Assistance, and Companionship; F: Flying User Interfaces.
% % \item \hfil $\feature0:\text{not relevant}$; $\feature1:\text{relevant}$; $\feature2:\text{relevant implicitly, partially, or in an emergent fashion}$.
% % {-} \or {$\bullet$} \or {$\circ$}
% \item \hfil {-}: not relevant; {$\bullet$}: relevant; {$\circ$}: relevant implicitly, partially, or in an emergent fashion.
% \item \hfil {CCC}: Communication, Control, and Comfort; {NAC}: Navigation, Assistance, and Companionship;
% \item \hfil {FUI}: Flying User Interfaces.
% \item \hfil {HCC}: Human-centered Concern; {DDC}: Drone Design Concern.
% \end{tablenotes} 
%\end{longtable}
\end{table*}

==> Brain_table.tex <==
\begin{table}[!Htb]
\caption{The overview of the Brain entity with the dimensions: EEG signals, preprocessing, signal acquisition, feature extraction, and feature classification methods identified in our corpus. Cont. next page.}
\small\sffamily\centering%
\begin{tabularx}{\linewidth}{l*{3}{X}c}
\specialrule{.2em}{.1em}{.1em}
\toprule
\thead{Dimension} & \thead{Sub-dimension}  & \thead{Number of Papers (\%)} & \thead{References} \\
\midrule
Signal Acquisition & Wired  &  21(24.1\%)  &      
\cite{ehrlich2019feasibility,kompatsiari2018,alimardani2022robotL,alimardani2020robotM,long2019eeg,chenga2023using,tang2022wearable,cao2018tactile,jo2022eeg,martinez2020non,zhang2021mind,sanguantrakul2020development,hernandez2019deep,gordleeva2020real,chen2020combination,quiles2022cross,ghosh2019continuous,kim2021affect,fang2022brain,lyu2022coordinating,richter2023eeg} \\
\addlinespace
                 & Wireless  & 46(52.9\%) & \cite{baka2019talking,belkacem2021cooperative,memar2018eeg,dissanayake2022eeg,chang2021eeg,aldini2019effect,toichoa2021emotion,staffa2022enhancing,wang2021focus,memar2019objective,lu2022online,ogino2018eeg,pawus2022application,cervantes2023cognidron,chu2018robot,kilmarx2018sequence,wang2018study,aldini2022detection,lu2020tractor,magee2021system,roshdy2021machine,aznan2019using,yu2019design,li2019hybrid,chiuzbaian2019mind,bahman2019robot,rashid2020investigating,guo2020nao,nann2020restoring,karunasena2021single,kuffuor2018brain,yuan2018brain,jiang2018brain,wang2018continuous,mondini2020continuous,araujo2021development,rahul2019eeg,ali2021eeg,shao2020eeg,boonarchatong2023green,prinsen2022passive,braun2019prototype,li2023act,qian2018affective,farmaki2022application,chhabra2020bci} \\
\addlinespace
                 & Not specified  & 20(23\%) &  \cite{iwane2019inferring,yoon2021effect,si2018towards,kar2021eeg,chen2021research,li2022eeg,roy2022classification,liu2021enhanced,abougarair2021implementation,du2021vision,penaloza2018android,ak2022motor,zhao2020multiple,korovesis2019robot,ai2018cooperative,wei2021control,francis2021eeg,xu2018eeg,wu2022deepbrain,sugiyama2023eeg}\\
\midrule
\midrule
Preprocessing  & ICA  &  3(3.4\%)  & \cite{dissanayake2022eeg,aldini2019effect,aldini2022detection} \\
\addlinespace
               & Band-pass filter & 59(67.8\%)  & \cite{belkacem2021cooperative,ehrlich2019feasibility,memar2018eeg,dissanayake2022eeg,aldini2019effect,staffa2022enhancing,iwane2019inferring,kompatsiari2018,memar2019objective,lu2022online,alimardani2022robotL,alimardani2020robotM,long2019eeg,yoon2021effect,chenga2023using,tang2022wearable,ogino2018eeg,pawus2022application,kar2021eeg,kilmarx2018sequence,wang2018study,cao2018tactile,li2022eeg,roy2022classification,jo2022eeg,aldini2022detection,martinez2020non,lu2020tractor,zhang2021mind,magee2021system,yu2019design,li2019hybrid,chiuzbaian2019mind,bahman2019robot,rashid2020investigating,zhao2020multiple,guo2020nao,gordleeva2020real,nann2020restoring,karunasena2021single,kuffuor2018brain,yuan2018brain,jiang2018brain,wang2018continuous,quiles2022cross,mondini2020continuous,wei2021control,araujo2021development,rahul2019eeg,francis2021eeg,shao2020eeg,prinsen2022passive,braun2019prototype,kim2021affect,qian2018affective,farmaki2022application,fang2022brain,lyu2022coordinating,richter2023eeg}
               \\
\addlinespace
               & Notch filter  & 13(14.9\%)   &  \cite{chu2018robot,roy2022classification,zhang2021mind,penaloza2018android,hernandez2019deep,li2019hybrid,gordleeva2020real,korovesis2019robot,kuffuor2018brain,yuan2018brain,chen2020combination,mondini2020continuous,farmaki2022application} \\
\addlinespace
               & Others  & 17(19.5\%)   &  \cite{baka2019talking,chang2021eeg,toichoa2021emotion,si2018towards,chen2021research,liu2021enhanced,abougarair2021implementation,du2021vision,roshdy2021machine,aznan2019using,sanguantrakul2020development,ai2018cooperative,ali2021eeg,boonarchatong2023green,li2023act,chhabra2020bci,wu2022deepbrain} \\
\addlinespace
               & Not mentioned & 6(6.9\%) & \cite{wang2021focus,cervantes2023cognidron,ak2022motor,ghosh2019continuous,xu2018eeg,sugiyama2023eeg} \\
\midrule
\midrule
Feature Extraction  & FT  &  12(13.8\%) & \cite{baka2019talking,wang2021focus,ogino2018eeg,chu2018robot,lu2020tractor,sanguantrakul2020development,hernandez2019deep,chiuzbaian2019mind,rashid2020investigating,korovesis2019robot,karunasena2021single,kuffuor2018brain} \\
\addlinespace
                 & WT & 9(10.3\%) & \cite{staffa2022enhancing,yoon2021effect,kar2021eeg,wang2018study,li2022eeg,lu2020tractor,zhao2020multiple,francis2021eeg,xu2018eeg} \\
\addlinespace
                 & CCA  & 4(4.6\%) & \cite{chen2021research,shao2020eeg,farmaki2022application,lyu2022coordinating} \\
\addlinespace
                 & CSP & 15(17.2\%) & \cite{long2019eeg,si2018towards,jo2022eeg,penaloza2018android,li2019hybrid,zhao2020multiple,guo2020nao,gordleeva2020real,kuffuor2018brain,jiang2018brain,wang2018continuous,ai2018cooperative,quiles2022cross,wei2021control,araujo2021development} \\
\addlinespace
                 & Others  &  45(51.7\%)  & \cite{belkacem2021cooperative,ehrlich2019feasibility,memar2018eeg,dissanayake2022eeg,chang2021eeg,aldini2019effect,toichoa2021emotion,iwane2019inferring,lu2022online,alimardani2022robotL,alimardani2020robotM,tang2022wearable,kilmarx2018sequence,cao2018tactile,roy2022classification,aldini2022detection,liu2021enhanced,martinez2020non,zhang2021mind,du2021vision,magee2021system,roshdy2021machine,aznan2019using,yu2019design,bahman2019robot,ak2022motor,nann2020restoring,yuan2018brain,chen2020combination,ghosh2019continuous,mondini2020continuous,rahul2019eeg,francis2021eeg,boonarchatong2023green,prinsen2022passive,braun2019prototype,li2023act,kim2021affect,qian2018affective,chhabra2020bci,richter2023eeg,jo2022eeg,guo2020nao,memar2019objective,chenga2023using} \\
\addlinespace
                & Not mentioned & 8(9.2\%) & \cite{kompatsiari2018,pawus2022application,cervantes2023cognidron,abougarair2021implementation,ali2021eeg,fang2022brain,wu2022deepbrain,sugiyama2023eeg} \\
\midrule
% \midrule
% Feature Classification & NN  &  17(19.5\%) & \cite{staffa2022enhancing,chenga2023using,tang2022wearable,pawus2022application,kar2021eeg,aldini2022detection,lu2020tractor,magee2021system,roshdy2021machine,aznan2019using,li2019hybrid,korovesis2019robot,ghosh2019continuous,rahul2019eeg,li2023act,fang2022brain,wu2022deepbrain} \\
% \addlinespace
%                  & LDA & 222(25.3\%) & \cite{belkacem2021cooperative,ehrlich2019feasibility,chang2021eeg,iwane2019inferring,si2018towards,kar2021eeg,chu2018robot,cao2018tactile,roy2022classification,jo2022eeg,aldini2022detection,rashid2020investigating,zhao2020multiple,gordleeva2020real,jiang2018brain,wang2018continuous,quiles2022cross,araujo2021development,xu2018eeg,braun2019prototype,farmaki2022application,lyu2022coordinating} \\
% \addlinespace
%                  & CCA  & 5(5.7\%) & \cite{chen2021research,zhang2021mind,du2021vision,yuan2018brain,chen2020combination} \\
% \addlinespace
%                  & SVM  & 13(14.9\%) & \cite{long2019eeg,ogino2018eeg,kar2021eeg,aldini2022detection,lu2020tractor,magee2021system,sanguantrakul2020development,rashid2020investigating,kuffuor2018brain,wei2021control,francis2021eeg,qian2018affective,chhabra2020bci} \\
% \addlinespace
%                  & Others  &  13(14.9\%)  & \cite{alimardani2022robotL,penaloza2018android,chiuzbaian2019mind,bahman2019robot,nann2020restoring,karunasena2021single,ai2018cooperative,kar2021eeg,aldini2022detection,rashid2020investigating,boonarchatong2023green,kim2021affect,richter2023eeg}\\
% \addlinespace
%                 & Not mentioned & 26(29.9\%) & \cite{baka2019talking,memar2018eeg,dissanayake2022eeg,aldini2019effect, toichoa2021emotion,wang2021focus,kompatsiari2018,memar2019objective,lu2022online,alimardani2020robotM,yoon2021effect,cervantes2023cognidron,kilmarx2018sequence,wang2018study,li2022eeg,liu2021enhanced,martinez2020non,abougarair2021implementation,hernandez2019deep,yu2019design,ak2022motor,mondini2020continuous,ali2021eeg,shao2020eeg,prinsen2022passive,sugiyama2023eeg} \\
% \bottomrule
% \specialrule{.2em}{.1em}{.1em}
\end{tabularx}
\label{tab:brain}
\end{table}

==> Brain_table_2.tex <==
\begin{table}[htb!]
\caption{Cont.}
\small\sffamily\centering%
\begin{tabularx}{\linewidth}{l*{3}{X}c}
\specialrule{.2em}{.1em}{.1em}
\toprule
\thead{Dimension} & \thead{Sub-dimension}  & \thead{Number of Papers (\%)} & \thead{References} \\
\midrule
% EEG Signals & First strategy  &  number  & Yes \\
%         & Second strategy  &   number   & No \\
%         & Second strategy  &   number   & No \\
% \midrule
% \midrule
% Signal Acquisition & Wired  &  21(24.1\%)  &      
% \cite{ehrlich2019feasibility,kompatsiari2018,alimardani2022robotL,alimardani2020robotM,long2019eeg,chenga2023using,tang2022wearable,cao2018tactile,jo2022eeg,martinez2020non,zhang2021mind,sanguantrakul2020development,hernandez2019deep,gordleeva2020real,chen2020combination,quiles2022cross,ghosh2019continuous,kim2021affect,fang2022brain,lyu2022coordinating,richter2023eeg} \\
% \addlinespace
%                  & Wireless  & 46(52.9\%) & \cite{baka2019talking,belkacem2021cooperative,memar2018eeg,dissanayake2022eeg,chang2021eeg,aldini2019effect,toichoa2021emotion,staffa2022enhancing,wang2021focus,memar2019objective,lu2022online,ogino2018eeg,pawus2022application,cervantes2023cognidron,chu2018robot,kilmarx2018sequence,wang2018study,aldini2022detection,lu2020tractor,magee2021system,roshdy2021machine,aznan2019using,yu2019design,li2019hybrid,chiuzbaian2019mind,bahman2019robot,rashid2020investigating,guo2020nao,nann2020restoring,karunasena2021single,kuffuor2018brain,yuan2018brain,jiang2018brain,wang2018continuous,mondini2020continuous,araujo2021development,rahul2019eeg,ali2021eeg,shao2020eeg,boonarchatong2023green,prinsen2022passive,braun2019prototype,li2023act,qian2018affective,farmaki2022application,chhabra2020bci} \\
% \addlinespace
%                  & Not specified  & 20(23\%) &  \cite{iwane2019inferring,yoon2021effect,si2018towards,kar2021eeg,chen2021research,li2022eeg,roy2022classification,liu2021enhanced,abougarair2021implementation,du2021vision,penaloza2018android,ak2022motor,zhao2020multiple,korovesis2019robot,ai2018cooperative,wei2021control,francis2021eeg,xu2018eeg,wu2022deepbrain,sugiyama2023eeg}\\
% \midrule
% \midrule
% Preprocessing  & ICA  &  3(3.4\%)  & \cite{dissanayake2022eeg,aldini2019effect,aldini2022detection} \\
% \addlinespace
%                & Band-pass filter & 59(67.8\%)  & \cite{belkacem2021cooperative,ehrlich2019feasibility,memar2018eeg,dissanayake2022eeg,aldini2019effect,staffa2022enhancing,iwane2019inferring,kompatsiari2018,memar2019objective,lu2022online,alimardani2022robotL,alimardani2020robotM,long2019eeg,yoon2021effect,chenga2023using,tang2022wearable,ogino2018eeg,pawus2022application,kar2021eeg,kilmarx2018sequence,wang2018study,cao2018tactile,li2022eeg,roy2022classification,jo2022eeg,aldini2022detection,martinez2020non,lu2020tractor,zhang2021mind,magee2021system,yu2019design,li2019hybrid,chiuzbaian2019mind,bahman2019robot,rashid2020investigating,zhao2020multiple,guo2020nao,gordleeva2020real,nann2020restoring,karunasena2021single,kuffuor2018brain,yuan2018brain,jiang2018brain,wang2018continuous,quiles2022cross,mondini2020continuous,wei2021control,araujo2021development,rahul2019eeg,francis2021eeg,shao2020eeg,prinsen2022passive,braun2019prototype,kim2021affect,qian2018affective,farmaki2022application,fang2022brain,lyu2022coordinating,richter2023eeg}
%                \\
% \addlinespace
%                & Notch filter  & 13(14.9\%)   &  \cite{chu2018robot,roy2022classification,zhang2021mind,penaloza2018android,hernandez2019deep,li2019hybrid,gordleeva2020real,korovesis2019robot,kuffuor2018brain,yuan2018brain,chen2020combination,mondini2020continuous,farmaki2022application} \\
% \addlinespace
%                & Others  & 17(19.5\%)   &  \cite{baka2019talking,chang2021eeg,toichoa2021emotion,si2018towards,chen2021research,liu2021enhanced,abougarair2021implementation,du2021vision,roshdy2021machine,aznan2019using,sanguantrakul2020development,ai2018cooperative,ali2021eeg,boonarchatong2023green,li2023act,chhabra2020bci,wu2022deepbrain} \\
% \addlinespace
%                & Not mentioned & 6(6.9\%) & \cite{wang2021focus,cervantes2023cognidron,ak2022motor,ghosh2019continuous,xu2018eeg,sugiyama2023eeg} \\
% \midrule
% \midrule
% Feature Extraction  & FT  &  12(13.8\%) & \cite{baka2019talking,wang2021focus,ogino2018eeg,chu2018robot,lu2020tractor,sanguantrakul2020development,hernandez2019deep,chiuzbaian2019mind,rashid2020investigating,korovesis2019robot,karunasena2021single,kuffuor2018brain} \\
% \addlinespace
%                  & WT & 9(10.3\%) & \cite{staffa2022enhancing,yoon2021effect,kar2021eeg,wang2018study,li2022eeg,lu2020tractor,zhao2020multiple,francis2021eeg,xu2018eeg} \\
% \addlinespace
%                  & CCA  & 4(4.6\%) & \cite{chen2021research,shao2020eeg,farmaki2022application,lyu2022coordinating} \\
% \addlinespace
%                  & CSP & 15(17.2\%) & \cite{long2019eeg,si2018towards,jo2022eeg,penaloza2018android,li2019hybrid,zhao2020multiple,guo2020nao,gordleeva2020real,kuffuor2018brain,jiang2018brain,wang2018continuous,ai2018cooperative,quiles2022cross,wei2021control,araujo2021development} \\
% \addlinespace
%                  & Others  &  45(51.7\%)  & \cite{belkacem2021cooperative,ehrlich2019feasibility,memar2018eeg,dissanayake2022eeg,chang2021eeg,aldini2019effect,toichoa2021emotion,iwane2019inferring,lu2022online,alimardani2022robotL,alimardani2020robotM,tang2022wearable,kilmarx2018sequence,cao2018tactile,roy2022classification,aldini2022detection,liu2021enhanced,martinez2020non,zhang2021mind,du2021vision,magee2021system,roshdy2021machine,aznan2019using,yu2019design,bahman2019robot,ak2022motor,nann2020restoring,yuan2018brain,chen2020combination,ghosh2019continuous,mondini2020continuous,rahul2019eeg,francis2021eeg,boonarchatong2023green,prinsen2022passive,braun2019prototype,li2023act,kim2021affect,qian2018affective,chhabra2020bci,richter2023eeg,jo2022eeg,guo2020nao,memar2019objective,chenga2023using} \\
% \addlinespace
%                 & Not mentioned & 8(9.2\%) & \cite{kompatsiari2018,pawus2022application,cervantes2023cognidron,abougarair2021implementation,ali2021eeg,fang2022brain,wu2022deepbrain,sugiyama2023eeg} \\
% \midrule
\midrule
Feature Classification & NN  &  17(19.5\%) & \cite{staffa2022enhancing,chenga2023using,tang2022wearable,pawus2022application,kar2021eeg,aldini2022detection,lu2020tractor,magee2021system,roshdy2021machine,aznan2019using,li2019hybrid,korovesis2019robot,ghosh2019continuous,rahul2019eeg,li2023act,fang2022brain,wu2022deepbrain} \\
\addlinespace
                 & LDA & 22(25.3\%) & \cite{belkacem2021cooperative,ehrlich2019feasibility,chang2021eeg,iwane2019inferring,si2018towards,kar2021eeg,chu2018robot,cao2018tactile,roy2022classification,jo2022eeg,aldini2022detection,rashid2020investigating,zhao2020multiple,gordleeva2020real,jiang2018brain,wang2018continuous,quiles2022cross,araujo2021development,xu2018eeg,braun2019prototype,farmaki2022application,lyu2022coordinating} \\
\addlinespace
                 & CCA  & 5(5.7\%) & \cite{chen2021research,zhang2021mind,du2021vision,yuan2018brain,chen2020combination} \\
\addlinespace
                 & SVM  & 13(14.9\%) & \cite{long2019eeg,ogino2018eeg,kar2021eeg,aldini2022detection,lu2020tractor,magee2021system,sanguantrakul2020development,rashid2020investigating,kuffuor2018brain,wei2021control,francis2021eeg,qian2018affective,chhabra2020bci} \\
\addlinespace
                 & Others  &  13(14.9\%)  & \cite{alimardani2022robotL,penaloza2018android,chiuzbaian2019mind,bahman2019robot,nann2020restoring,karunasena2021single,ai2018cooperative,kar2021eeg,aldini2022detection,rashid2020investigating,boonarchatong2023green,kim2021affect,richter2023eeg}\\
\addlinespace
                & Not mentioned & 26(29.9\%) & \cite{baka2019talking,memar2018eeg,dissanayake2022eeg,aldini2019effect, toichoa2021emotion,wang2021focus,kompatsiari2018,memar2019objective,lu2022online,alimardani2020robotM,yoon2021effect,cervantes2023cognidron,kilmarx2018sequence,wang2018study,li2022eeg,liu2021enhanced,martinez2020non,abougarair2021implementation,hernandez2019deep,yu2019design,ak2022motor,mondini2020continuous,ali2021eeg,shao2020eeg,prinsen2022passive,sugiyama2023eeg} \\
\bottomrule
\specialrule{.2em}{.1em}{.1em}
\end{tabularx}
\label{tab:brain2}
\end{table}
